Self-Awareness of Cloud Applications

Cloud applications today deliver an increasingly larger portion of the Information and Communication Technology (ICT) services. To address the scale, growth, and reliability of cloud applications, self-aware management and scheduling are becoming commonplace. How are they used in practice? In this chapter, we propose a conceptual framework for analyzing state-of-the-art self-awareness approaches used in the context of cloud applications. We map important applications corresponding to popular and emerging application domains to this conceptual framework, and compare the practical characteristics, benefits, and drawbacks of self-awareness approaches. Last, we propose a roadmap for addressing open challenges in self-aware cloud and datacenter applications.

==> sections/approaches-metaheuristic.tex <==

\subsection{Meta-heuristic optimization}\label{sec:7_2_generalapproaches:metaheuristic}

\comment{(Should this be merged with number 7?)}
\comment{ Arif merged this with approaches-constraints.tex, commented
  out link from approaches.tex.}
\comment{(DONE) AP(Arif)}


{\bf Description:}
- overview of what the technique is about. (possible contrast with non-self-aware approaches)


{\bf Expected Impact:}
- describe main promise of the technique
- link back to applications (and metrics) in Section 3. List all application types to which this technique has already been applied, if you have references.
- link back to problems in Section 4.


{\bf Details:}
- details 

{\bf Use Cases:}
- give 1-2 examples


		Example problems: dynamic load balancing
{\bf REF:Kimberly Keeton, Dirk Beyer, Ernesto Brau, Arif Merchant, Cipriano A. Santos, Alex Zhang. On the road to recovery: restoring data after disasters. Eurosys 2006.}
\url{http://doi.acm.org/10.1145/1217935.1217958}

{\bf REF: Shravan Gaonkar, Kimberly Keeton, Arif Merchant, William H. Sanders. Designing Dependable Storage Solutions for Shared Application Environments. IEEE Trans. Dependable Sec. Comput., vol. 7 (2010), pp. 366-380.}
\url{https://www.perform.illinois.edu/Papers/USAN_papers/07GAO02.pdf}



==> sections/approaches-recovery.tex <==

%Vehicles, as they are becoming increasingly endowed with computation and communication technologies, are a prime example of the
% need for troubleshooting within a cyber-physical application (see 
%Section~\ref{sec:7_2_generalapplications_cyberphysical}).  
%Both autonomous and semi-autonomous vehicles could benefit 
%much from being carefully orchestrated 
%and controlled by means of shared information resources that reflect the physical world, for example weather maps, traffic maps,
% and so forth. 
%With less human involvement and situation awareness on-board vehicles, how to act in off-nominal situations also becomes more
% challenging. In this context, improved 
%system health management, including diagnostics and prognostics capabilities 
%\cite{mengshoel10probabilistic,schumann13software,schumann2013towards,ricks13diagnosis}, on-board autonomous and semi-autonomous %vehicles is important. The goal is to improve the on-board sensing, perception, and cognition capabilities, and also improve 
%communication through a centralized or distributed cloud.  







==> sections/problems-deployment.tex <==

\subsection{ (Re-Configuration and Dynamic Load Balancing} \label{sec:7_2_generalproblems:deployment}

\comment{(TODO) AP(Eva): describe. Note from Alex: added a few words about architectural (re)configuration, where queues are (dynamically) configured, and load sharing between queues is (dynamically) configured.}

{\bf Context:} 
For many of the application types we describe in Section~\ref{sec:7_2_generalapplications}, the condition they are operating under can change 

{\bf Problem:}
%- the problem/the difficulty/the challenge:
Related to autoscaling (Section~\ref{sec:7_2_generalproblems:autoscaling}, which keeps the same architecture while changing the scale of the system, architectural reconfiguration is a family of techniques that reconfigure the entire architecture of the system. The main targets for reconfiguration are the queues and the load sharing between queues.
When changes in the workload occur, the current architecture of the system may become obsolete, even if individual components are equipped with self-awareness techniques. For example, even if individual virtual clusters can auto-scale, the overall architecture in which the virtual clusters are deployed on the same physical infrastructure would also need self-aware capabilities.
A self-aware architecture should reconfigure and manage its components, for example by resizing its queues and by changing their scheduling policies, or by changing the paths for sharing load between queues.

For dynamic load balancing, the challenges include how to quantify load imbalance, how to weigh the cost vs. the benefit of remedial actions such as VM migrations, and how to deak with the tradeoff between faster response and stability.

{\bf Expected Advancement:}
- what advancement is needed to solve the problem? what should be done? (is there an expected range for the advancement?)


{\bf Expected Impact on Application Types:}
%- which applications, from our list, will be affected? (is there an expected impact?)
Especially batch processing, either compute-intensive (Section~\ref{sec:7_2_generalapplications_batch}) or data-intensive (Section~\ref{sec:7_2_generalapplications_dataintensive}), and data-stream processing (Section~\ref{sec:7_2_generalapplications_datastream}).

For applications running on virtualized infrastructure that can be migrated at runtime, better load balance across a cluster of servers can improve application ``happinesss". For example, VMware Distributed Resource Scheduler (DRS)~\cite{Gulati:VMTJ:2012} manages a set of virtual machines running on a cluster of physical hosts and performs dynamic load balancing to avoid hot spots and improve VM performance.

\comment{(TODO) AP(Alex) Move the paper to the ref. section, and provide a description in this subsection.}
{\bf REF: Bogdan Ghit, Nezih Yigitbasi, Alexandru Iosup, and Dick H. J. Epema: Balanced resource allocations across multiple dynamic MapReduce clusters. SIGMETRICS 2014: 329-341} \url{http://pds.twi.tudelft.nl/~iosup/dynamic-mapreduce14sigmetrics.pdf}
